Prototypical Description and Controller Design for a Set of Systems Using v-gap Based Clustering

We present an approach to design stabilizing controllers for a set of linear systems without restrictions regarding their modeling order. To this end, the systems are treated as abstract objects in the space of the $\nu$-gap metric. Via a cluster analysis the set of systems is split into v-gap similar clusters which are treated separately. For this purpose we provide an algorithm that constructs an explicit prototype system by generalizing the information of a given set of systems. Applying this algorithm to each cluster a set of prototype systems is obtained. Given these prototypes we design controllers in such a way that all systems assigned to a cluster will be stabilized by a corresponding controller. The approach is demonstrated for a set of 80 linear systems.

==> ACSD-preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACSD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Packages
\usepackage{xspace}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{cite}
\usepackage{nicefrac}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsthm}

%%%% Arrows
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\la}{\leftarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\LRa}{\LeftRightarrow}

%%%% Theorems
%\newtheorem{dfn}{Definition}
%\newtheorem{asm}{Assumption}
%\newtheorem{fct}{Fact}
%\newtheorem*{fct*}{Fact}
%\newtheorem{prp}{Proposition}
%\newtheorem*{prp*}{Proposition}
%\newtheorem{lem}{Lemma}
%\newtheorem*{lem*}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{crl}{Corollary}
%\newtheorem*{crl*}{Corollary}
%\newtheorem{rem}{Remark}
%\newtheorem*{rem*}{Remark}
%\newtheorem{exm}{Example}
%\newtheorem*{exm*}{Example}
%\newtheorem{prb}{Problem}
%\newtheorem*{prb*}{Problem}

%%%% Abbreviations
\newcommand{\ie}{\unskip, i.\,e.,\xspace}
\newcommand{\eg}{\unskip, e.\,g.,\xspace}
\newcommand{\pd}{p.\,d.\xspace}
\newcommand{\sut}{\text{s.\,t.\,}}
\newcommand{\wrt}{w.\,r.\,t.\xspace}
\newcommand{\rt}{r.\,t.\xspace}

%%%% Sets
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}

\newcommand{\sm}{\ensuremath{\setminus}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%% Texts
\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\dom}{\ensuremath{\text{dom}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\co}{\ensuremath{\text{co}}}
\newcommand{\cco}{\ensuremath{\overline{\text{co}}}}

%%%% Fonts
\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\ii}[1]{\textit{#1}}
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}

%%%% Symbols
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\pdiff}[2]{ \ensuremath{ \frac{\partial {#1}}{\partial {#2}} } }
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\ball}{\ensuremath{\mathcal B}}
\newcommand{\tp}{^{\top}}			% Transpose
\newcommand{\D}{\ensuremath{\mathcal{D}}}		% Generalized derivative
\newcommand{\K}{\ensuremath{\mathcal{K}}\xspace}		% Capital kappa
\newcommand{\KL}{\ensuremath{\mathcal{KL}}\xspace}		% Kappa-ell
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}\xspace}		% Kappa-infinity
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argsup}{arg\,sup}

%%%% References
\newcommand{\reffig}[1]{Fig.\,\ref{#1}}  
%\newcommand{\refFig}[1]{Figure\, \ref{#1}} 

%%%% Wraps
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\scal}[1]{\left\langle#1\right\rangle}

%%%% Probability
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}

%%%% Review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{\textcolor{dgreen}{#1}}

%%%% Miscellaneous
\newcommand{\spc}{\ensuremath{\,\,}}	% Logical formula separator

%%%% Environments
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Prototypical Description and Controller Design for a Set of Systems Using v-gap Based Clustering/ACSD-preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACSD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Packages
\usepackage{xspace}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{cite}
\usepackage{nicefrac}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsthm}

%%%% Arrows
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\la}{\leftarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\LRa}{\LeftRightarrow}

%%%% Theorems
%\newtheorem{dfn}{Definition}
%\newtheorem{asm}{Assumption}
%\newtheorem{fct}{Fact}
%\newtheorem*{fct*}{Fact}
%\newtheorem{prp}{Proposition}
%\newtheorem*{prp*}{Proposition}
%\newtheorem{lem}{Lemma}
%\newtheorem*{lem*}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{crl}{Corollary}
%\newtheorem*{crl*}{Corollary}
%\newtheorem{rem}{Remark}
%\newtheorem*{rem*}{Remark}
%\newtheorem{exm}{Example}
%\newtheorem*{exm*}{Example}
%\newtheorem{prb}{Problem}
%\newtheorem*{prb*}{Problem}

%%%% Abbreviations
\newcommand{\ie}{\unskip, i.\,e.,\xspace}
\newcommand{\eg}{\unskip, e.\,g.,\xspace}
\newcommand{\pd}{p.\,d.\xspace}
\newcommand{\sut}{\text{s.\,t.\,}}
\newcommand{\wrt}{w.\,r.\,t.\xspace}
\newcommand{\rt}{r.\,t.\xspace}

%%%% Sets
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}

\newcommand{\sm}{\ensuremath{\setminus}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%% Texts
\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\dom}{\ensuremath{\text{dom}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\co}{\ensuremath{\text{co}}}
\newcommand{\cco}{\ensuremath{\overline{\text{co}}}}

%%%% Fonts
\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\ii}[1]{\textit{#1}}
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}

%%%% Symbols
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\pdiff}[2]{ \ensuremath{ \frac{\partial {#1}}{\partial {#2}} } }
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\ball}{\ensuremath{\mathcal B}}
\newcommand{\tp}{^{\top}}			% Transpose
\newcommand{\D}{\ensuremath{\mathcal{D}}}		% Generalized derivative
\newcommand{\K}{\ensuremath{\mathcal{K}}\xspace}		% Capital kappa
\newcommand{\KL}{\ensuremath{\mathcal{KL}}\xspace}		% Kappa-ell
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}\xspace}		% Kappa-infinity
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argsup}{arg\,sup}

%%%% References
\newcommand{\reffig}[1]{Fig.\,\ref{#1}}  
%\newcommand{\refFig}[1]{Figure\, \ref{#1}} 

%%%% Wraps
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\scal}[1]{\left\langle#1\right\rangle}

%%%% Probability
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}

%%%% Review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{\textcolor{dgreen}{#1}}

%%%% Miscellaneous
\newcommand{\spc}{\ensuremath{\,\,}}	% Logical formula separator

%%%% Environments
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
